Usability of Privacy Controls in Top Health Websites

With the increasing awareness and concerns around privacy, many service providers offer their users various privacy controls. Through these controls, users gain greater authority over the collection, utilisation, and dissemination of their personal information by the services. However, these controls may be buried deep within menus or settings, making them difficult for a user to access. Additionally, the terminology used to describe privacy controls can sometimes be confusing or technical, further complicating the user's ability to understand and use them effectively. This is especially true for health websites, as users often share sensitive information about their health and well-being. While many privacy controls have been proposed to protect user data on these sites, existing research focuses on individual controls (e.g., privacy policies or cookie opt-outs) rather than providing a comprehensive overview of the privacy landscape. In addition, many studies concentrate on the technical aspects of privacy controls without considering the usability of these features from a user's perspective. This paper aims to fill the gaps in the existing work by analysing four privacy controls, namely privacy nudge, privacy notice, privacy policy, and privacy setting, and evaluating their usability on the top 100 most visited health websites. First, we define usability attributes for each privacy control in three website visit scenarios; the guest, registering, and log-in visits. These attributes include awareness, efficiency, comprehension, functionality, and choice. Then, we design a survey template based on these attributes and scenarios and collect data about privacy controls. Next, we analyse the availability and usability of each privacy control on health websites. Finally, we provide suggestions for improving the design of these privacy controls based on the data analysis results.

==> Sections/Analysis.tex <==

\section{Survey Data Analysis}
\label{sec:analysis}

\subsection{Privacy Control Design Suggestions}
\subsubsection{How to Combine Privacy Controls}
We researched four privacy controls. The privacy notice and privacy policy give users the right to know, focusing on delivering privacy-related information. On the other hand, the privacy nudge and privacy setting provide users the freedom of choice, which require users' consent or selection. According to the requirement of GDPR and CCPA, the most basic and core rights to users are the right to know and the right to choose (e.g., consent or opt-out). In addition, Art. 9 GDPR states that processing of data concerning health shall be prohibited unless the data subject has given explicit consent to the processing of those personal data. Therefore, health websites have higher requirements for privacy controls. We will discuss the combination of these privacy controls to deliver these rights to users in different visit scenarios.
\paragraph{Guest Visit Scenario} 
For users' right to know, the privacy policy comprehensively describes a website's privacy practices. Therefore, a website's privacy policy is mandatory in any visit scenario. In the guest visit scenario, even though users have not left many browsing traces and personally identifiable information on websites in a guest visit scenario, websites need to provide users with timely notice, at or before the point of collection, according to the requirement of CCPA. Therefore, more than a privacy policy is needed to meet the timely notice requirement. For example, we need an intrusive privacy nudge or notice to attract the users' attention and inform them of the privacy policy and other privacy practices. For users' right to choose, both the privacy nudge and setting can provide users with the option to choose based on their preferences. Still, they each have their own advantages, e.g., the privacy nudge is salient, and the privacy setting can be accessible at any time.

To summarize, the minimum combination of privacy controls includes the privacy policy and the privacy nudge (intrusive style and contains customized options), or the privacy policy (contains setting options, links, or clear setting guidance) and the privacy nudge/notice (intrusive style). The best combination of privacy controls consists of the privacy policy, the privacy nudge (intrusive type and has customized options or privacy setting link), and the privacy setting.
\paragraph{Registering Scenario}
According to the notice requirement of CCPA,  websites shall provide new notice at or before data collection when they plan to collect additional categories of personal information. In the registering process, users need to share more personal information with websites than the guest visit scenario, like name, phone number, email, and residence address. Therefore, websites still need to provide the notice during registration. The combination is the same as the guest visit scenario except that the privacy nudge/notice is not required to be the intrusive type for the minimum configuration because check box content or plain text nearby the sign-up button is also obvious and will not be ignored. 
\paragraph{Log-in visit Scenario}
Differently from the other two visit scenarios, users should have been aware of and consented to the privacy practices of this website. Therefore, the minimum configuration can only include the privacy policy (contains setting options, links, or clear setting guidance) and the best combination includes the privacy policy and the privacy setting.

According to the analysis of Section~\ref{availability}, we learned the current availability of privacy controls on health websites and the gap between reality and expectations. The privacy policy is available for almost all websites, but the availability of the privacy nudge, privacy notice, and privacy setting is deficient, especially in the guest visit scenario. More websites implement the privacy nudge and notice in the registering scenario than in the guest visit scenario. We recalculate the availability of the combination of privacy controls in Table~\ref{table:availability_best_mini}.
The websites that can meet the minimum requirement in three visit scenarios account for 26.0\%, 57.1\%, and 69.0\%. The ratios of the best configuration are much lower. In addition, we note that the regulatory compliance of the websites with the minimum configuration is over 80.0\%. That means the regulations guide the design of a website, especially GDPR and CCPA.  

In summary, we suggest website designers increase the privacy controls according to the best configuration (at least the minimum configuration), especially improving the privacy controls of the guest visit scenario. Considering the binding effect of regulations on website design, we suggest the counties of the Asia-Pacific region (see Figure~\ref{region}) build their privacy protection regulations or follow GDPR or CCPA, which contribute significantly to the availability of privacy controls.
\begin{table}
\caption{The Count for Websites With Different Privacy Control Configuration and Their Regulation Compliance}
\label{table:availability_best_mini}
\footnotesize
\centering
\begin{tabular}{  cccc }
\toprule
\textbf{Scenario}&\textbf{Minimum Configuration}&\textbf{Best Configuration}&\textbf{Regulatory Compliace}\\ %&\textbf{Regulation Compl. (Best)} \\
\midrule
Guest Visit (100 total) &26 &13 & 80.8\% (21/26)\\ %&84.6\% (11/13)  \\
Registering (42 total) &24 &2 &87.5\% (21/24) \\% &50.0\% (1/2) \\
Log-in Visit (42 total) &29 &21 & 89.7\%(26/29) \\ %& 81.0\%(17/21) \\
\bottomrule
\end{tabular}
\end{table}


\subsubsection{How to Design Privacy Controls}
In this section, we will discuss how to improve the usability of each privacy control based on our previous analysis in Section~\ref{usability_analysis}.
\paragraph{Privacy Nudge and Notice}
\paragraph{Awareness} According to the analysis about the privacy nudge and notice in Section~\ref{nudge_analysis} and ~\ref{notice_analysis}, 82.0\%  and 94.0\% of websites do not have or only have subtle privacy nudges and notice in the guest visit scenario. Therefore website designers need to introduce salient privacy nudges or notices to improve the awareness of privacy information. Specifically, using intrusive display types like `Pop-up Window' and `Banner' (`Pop-up Window' is better) and consistent display locations like middle or top. Full-screen privacy nudges/notices occupy users' entire field of view and would be the best way to display the privacy nudge/notice. 

In the registering scenario,  92.3\% of privacy nudges are displayed nearby the sign-up button as check box content or with a full-screen new page. The display location and type are acceptable because a user needs to click the check box or close the new page to finish the registration. For privacy notice, most of them display as the ‘Plant Text’ (85.2\%) located nearby sign up/log-in/subscribe buttons which is not intrusive style and can be easily ignored
because whether you read the plain text will not affect your registration. Only 2 out of 27 privacy notices
displayed obviously. We suggest the privacy notice also utilize a `Pop-up Window' (located at the top or middle) or full-Screen new page to deliver privacy information as in the guest visit scenario.

\paragraph{Choice} 
To respect users' right to choose, we suggest that the privacy nudge should contain `Accept', `Reject' and `Manage' options and explain the meaning of selecting each option. This will ensure that the decisions made by users follow their true intentions. We checked our survey results and found that only 10.0\% (10 out of 100) and none of the websites meet this design requirement in the guest visit and registering scenario, respectively. Therefore, most websites need improvement in this aspect. 

\paragraph{Functionality} Previous analysis showed that most privacy nudges/notices only cover one or two types of privacy content (i.e., functions), like cookie and privacy policy. Which functions should be covered depends on what data the website plans to collect. The fifth clause of 999.305 b) in CCPA states that `business shall not collect categories of personal information other than those disclosed in the notice at collection.'  Based on this design principle and the analysis results (popularity of each function), we suggest the privacy nudge/notice in the guest visit scenario contains `Cookie', `Privacy Policy', `Location', and `Advertisement'. `Privacy Policy' is the overall description of the privacy practice of a website, and it is mandatory to cover. In addition, websites can easily collect users' browsing `Cookie' and `Location' without the user being aware of them. Therefore, it is reasonable to contain these two functions. `Advertisement' is related to `Cookie' and selling information to the third party, which we also suggest covering. The other three functions, `Email/Notification', `Profile/PII', and `History', are usually shared by users voluntarily and are not as necessary as those.
In the registering scenario, we do not need to repeat the functions provided in the guest visit scenario except `Privacy Policy' because it can provide users overall view of the privacy practices. Apart from `Privacy Policy', we suggest the privacy nudge/notice contain `Email/Notification' and `Profile/PII' as the basic configuration because we usually need to provide such personal information during registration. Other specific information like `History' should be added to the basic configuration according to a website's service.

\paragraph{Privacy Policy}
\paragraph{Awareness} According to the analysis results in Section~\ref{policy_analysis}, most privacy policies are located at the homepage footer in the guest visit scenario and displayed as links in privacy notices/nudges in the registering scenario. Consistent display location facilitates users' access to the privacy policy. Therefore, we have few improvement suggestions for the display of a privacy policy. The only advice for the registering scenario is to provide a privacy policy link in a privacy nudge rather than a privacy notice that is easily ignored. Alternatively, we suggest displaying a privacy policy with a full-screen new page to attract users' attention to the maximum extent.

\paragraph{Efficiency} 
Most privacy policies can be accessed with two clicks (i.e., scrolling down and a click on the privacy policy button). A higher efficient way is leveraging privacy nudge/notice to access the privacy policy with only one click. According to our privacy control design suggestions about the combination of privacy controls and the privacy nudge/notice functionality, websites that meet our recommendations can achieve the highest efficiency access. 

\paragraph{Comprehension}
In Section~\ref{policy_analysis}, we utilize whether it contains various languages and the table of content as two features to evaluate the comprehension of a privacy policy. Our targeted 100 health websites are from 21 countries and with about 14 languages. Over three-quarters of privacy policies do not provide different language versions, but we can read them utilizing the translate tool of a browser (i.e., Chrome). Therefore, we recommend that the Privacy Policy be made available in multiple languages based on the potential user's first language to help users understand it. It is also acceptable to display the privacy policy in HTML formatted pages rather than PDF or other embedded text that cannot be translated automatically. While automatic translation is inaccurate, it will allow the website to match as many users as possible.
From the survey results, 76.8\% of privacy policies do not provide the table of content. The privacy policy is usually very long, for example, the website `familyandpets.com' has a privacy policy over thirty pages. It's easy for users to get lost in the lengthy text without the table of content. Therefore, we suggest the privacy policy to provide the table of content because it can help users have a comprehensive understanding of the privacy policy and quickly locate the parts they care about.

\paragraph{Choice}
The previous analysis noted that 36 out of 99 privacy policies neither provide privacy setting links nor clear privacy setting guidance. According to the privacy control combination proposed before, privacy setting is essential to meet users' right to choose. We recommend the privacy policy provide customized privacy setting links where users can access all the privacy options with concise explanations and do not need to find the dispersed third-party links. Third-party privacy setting interfaces, like cookie opt-out web pages, are usually hard to understand and to choose based on users' real intentions. Alternatively, the privacy policy can meet the users' right to choose by clearly guiding the privacy setting (e.g., step by step) and combining with third-party links (with instructions for use).

\paragraph{Privacy Setting}
\paragraph{}
In line with the previous result analysis, our design suggestions for privacy settings are organized from the perspective of different visit scenarios.

\paragraph{Guest Visit Scenario}
According to the suggestion for the combination of privacy controls in the guest visit scenario. The best configuration should contain the privacy policy, privacy nudge (intrusive type and has customized options or privacy setting link), and privacy setting. That means it is better to display the privacy setting as a button at the footer and as options or a link in the privacy nudge. Currently, in the survey results, we found that only 7.0\% of websites contain both display types of privacy settings and 76.5\% privacy settings appear at the homepage footer. Therefore, to draw more attention from users, we suggest adding setting options or the setting link to the privacy nudge. In addition, to improve the access efficiency (only 14.7\% one-click access), directly linking to the privacy setting from the privacy nudge is the best method. About the comprehension attribute, only 11.8\% of privacy settings provide additional languages. However, most of these privacy settings can be translated automatically, which is still acceptable. Moreover, regarding to the functionality, 58.8\% of privacy settings only cover one function. Our suggestion for functionalities of the privacy setting is similar to the privacy nudge, covering `Cookie', `Location', and `Advertisement' (only excluding `Privacy Policy').

\paragraph{Registering Scenario}
From previous analysis results, we note that the display location and type of the privacy setting in the registering scenario has no obvious pattern. We suggest to provide check box content (containing the privacy setting link) nearby the sign-up button or a full screen privacy setting page after clicking the sign-up button to ensure this privacy control is available before information collection and is salient for users. Regarding to the comprehension attribute, it is better to provide a privacy setting with multi-language versions or at least make the privacy setting page can be automatically translated by the browser. Furthermore, most privacy settings only cover one function `Cookie’. We recommend that the privacy setting should cover `Email/Notification’ and `Profile/PII’ because users usually need to share email, phone number and other PII information with the website during registration. `Cookie' and `Location' are not necessary if the privacy setting of the guest visit scenario has covered them.

\paragraph{Log-in Visit Scenario}
In the log-in visit scenario, the privacy setting is a part of the account setting, where users can set or change their settings. Therefore, the location should be fixed and easy to find, and the functionality should cover the full range.
Currently, 90.9\% of the account privacy settings are located at the header, and 81.6\% can be accessed within three clicks (included). Regarding comprehension, the situation is the same as the other two scenarios. Thus we only give suggestions about the functionality, covering `Cookie', `Advertisement', `Location', `Email/Notification’, `Profile/PII’, and certain functions like `History' and `Activity' based on a website's service.
